FM-SIREN & FM-FINER: Implicit Neural Representation Using Nyquist-based Orthogonality

Existing periodic activation-based implicit neural representation (INR) networks, such as SIREN and FINER, suffer from hidden feature redundancy, where neurons within a layer capture overlapping frequency components due to the use of a fixed frequency multiplier. This redundancy limits the expressive capacity of multilayer perceptrons (MLPs). Drawing inspiration from classical signal processing methods such as the Discrete Sine Transform (DST), in this paper, we propose FM-SIREN and FM-FINER, which assign Nyquist-informed, neuron-specific frequency multipliers to periodic activations. Contrary to existing approaches, our design introduces frequency diversity without requiring hyperparameter tuning or additional network depth. This simple yet principled approach reduces the redundancy of features by nearly 50% and consistently improves signal reconstruction across diverse INR tasks, such as fitting 1D audio, 2D image and 3D shape, and video, outperforming their baseline counterparts while maintaining efficiency.

==> additional_sections/NeRF.tex <==
\subsection{Neural Radiance Fields}

\par NeRF synthesizes novel 3D scene views from sparse 2D images by learning a continuous volumetric representation optimized via ray-based rendering \cite{mildenhall2020nerfrepresentingscenesneural}. In our experiments, the volume is discretized at a resolution of $100 \times 100 \times 100$, corresponding to a Nyquist frequency of $50$ cycles/volume. We adopt the concise implementation of \cite{vandegar2025nerf100lines} on the Blender dataset \cite{mildenhall2021nerf}, using networks with five layers that model density and color. Performance is evaluated as the average PSNR across all 200 test images per scene, each at a resolution of $400 \times 400$. As reported in Table~\ref{tab:NeRF} and illustrated in Figure~\ref{fig:NeRF}, FM-SIREN and FM-FINER achieve higher PSNR than baseline models in most scenes. Although the improvements in reconstruction quality are modest, both FM-SIREN and FM-FINER reduce compute time by $14.53\%$ and $17.06\%$, respectively, demonstrating the efficiency gains of our approach.


\begin{figure}[t]
    \centering
    % Row 1
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/NeRF/GT_NeRF_chair.pdf}
        \caption{Ground Truth}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/NeRF/SIREN_NeRF_chair.pdf}
        \caption{SIREN}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/NeRF/FINER_NeRF_chair.pdf}
        \caption{FINER}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/NeRF/PE_NeRF_chair.pdf}
        \caption{PE}
    \end{subfigure}

    % Row 2
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/NeRF/Gauss_NeRF_chair.pdf}
        \caption{GAUSS}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/NeRF/WIRE_NeRF_chair.pdf}
        \caption{WIRE}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/NeRF/eSIREN_NeRF_chair.pdf}
        \caption{FM-SIREN}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/NeRF/eFINER_NeRF_chair.pdf}
        \caption{FM-FINER}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Qualitative reconstruction results of the Chair scene from the Blender dataset \cite{mildenhall2021nerf}, using five-layer networks (three layers for the first block, one layer for density, and one layer for color). FM-SIREN and FM-FINER achieve improvements over the baselines, with exact PSNR values reported in Table~\ref{tab:NeRF}.}
    \vspace{-10pt}

    \label{fig:NeRF}
\end{figure}


\begin{table}[h!]
    \centering
    \caption{Epoch time, number of parameters, and PSNR for NeRF fitting on the Blender dataset \cite{mildenhall2021nerf}. \colorbox{Goldenrod}{Best} and \colorbox{Dandelion}{Second Best} results are highlighted.}
    \vspace{-5pt}
    \resizebox{1\textwidth}{!}{%
    \begin{tabular}{@{}lc ccccccccc@{}}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & 
        \multirow{2}{*}{\textbf{Epoch Time (s)}} & 
        \multirow{2}{*}{\textbf{Parameters}} & 
        \multicolumn{8}{c}{\textbf{PSNR} $\uparrow$} \\
        \cmidrule(lr){4-11}
         & & & \textbf{Lego} & \textbf{Ship} & \textbf{Chair} & \textbf{Mic} & \textbf{Materials} & \textbf{Hotdog} & \textbf{Ficus} & \textbf{Drums} \\
        \midrule
        FINER & $106.84$ & $199,428$ & \colorbox{Dandelion}{$28.01$} & $33.09$ & $34.53$ & $34.44$ & $33.38$ & $37.16$ & $33.75$ & $32.51$ \\
        GAUSS & $98.68$ & $199,428$ & $27.58$ & $32.91$ & $34.23$ & \colorbox{Dandelion}{$34.48$} & $33.21$ & $36.66$ & $33.33$ & $32.31$ \\
        Positional Encoding & $126.33$ & $214,788$ & $27.63$ & $32.48$ & $34.13$ & $34.24$ & $32.86$ & $36.17$ & $32.82$ & $31.72$ \\
        SIREN & $122.12$ & $199,428$ & $27.81$ & $33.08$ & $34.42$ & $34.45$ & $33.38$ & $37.00$ & \colorbox{Goldenrod}{$33.79$} & $32.48$ \\
        WIRE & $140.04$ & $199,428$ & $23.36$ & $20.34$ & $25.21$ & $26.31$ & $23.07$ & $27.50$ & $23.19$ & $21.11$ \\
        \midrule
        \textbf{FM-SIREN} & $104.37$ & $199,428$ & $27.55$ & \colorbox{Goldenrod}{$33.17$} & \colorbox{Dandelion}{$34.55$} & \colorbox{Goldenrod}{$34.64$} & \colorbox{Goldenrod}{$33.45$} & \colorbox{Dandelion}{$37.37$} & \colorbox{Dandelion}{$33.76$} & \colorbox{Goldenrod}{$32.54$} \\
        \textbf{FM-FINER} & $88.61$ & $199,428$ & \colorbox{Goldenrod}{$28.11$} & \colorbox{Dandelion}{$33.14$} & \colorbox{Goldenrod}{$34.56$} & $29.81$ & \colorbox{Dandelion}{$33.41$} & \colorbox{Goldenrod}{$37.41$} & $33.73$ & \colorbox{Dandelion}{$32.53$} \\
        \bottomrule
    \end{tabular}%
    }
    \label{tab:NeRF}
\end{table}

==> additional_sections/audio.tex <==
\subsection{Audio Fitting}
\vspace{-8pt}
\begin{figure}[t]
    \centering
    % Row 1
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/audio/GT_audio.pdf}
        \caption{Ground Truth}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/audio/SIREN_audio.pdf}
        \caption{SIREN}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/audio/FINER_audio.pdf}
        \caption{FINER}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/audio/PE_audio.pdf}
        \caption{PE}
    \end{subfigure}

    % Row 2
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/audio/Gauss_audio.pdf}
        \caption{GAUSS}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/audio/WIRE_audio.pdf}
        \caption{WIRE}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/audio/eSIREN_audio.pdf}
        \caption{FM-SIREN}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{figures/experimental_results/audio/eFINER_audio.pdf}
        \caption{FM-FINER}
    \end{subfigure}

    \caption{Qualitative results of one-second audio reconstructions for the 1995 Pacific Grand Prix clip in the Spoken English Wikipedia dataset \cite{spokenwikipedia}, using two-layer networks with different approaches. The one-second MSE of each reconstruction is reported in the top-right corner of its subfigure. FM-SIREN and FM-FINER achieve visibly closer alignment to the ground truth and substantially lower MSE compared to the baselines. \colorbox{red}{\textcolor{white}{Red}}, \colorbox{customblue}{\textcolor{white}{medium blue}}, and \colorbox{black}{\textcolor{white}{black}} lines correspond to ground truth, reconstructed signal, and error signal, respectively.}

    \label{fig:audio-fit}
\end{figure}

\begin{table}[t]
    \centering
    \caption{\label{fig:AudioMse} Average MSE for audio fitting on the Spoken English Wikipedia dataset \cite{spokenwikipedia}, comparing different INR models. \colorbox{Goldenrod}{Best} and \colorbox{Dandelion}{Second Best} results are highlighted.}
    \vspace{-5pt}
    \resizebox{1\textwidth}{!}{%
    \begin{tabular}{lccccc|cc}
        \toprule
        \textbf{Model} & FINER & GAUSS & PE & SIREN & WIRE & \textbf{FM-SIREN} & \textbf{FM-FINER} \\
        \midrule
        \textbf{MSE} $\downarrow$ & $2.631 \times 10^{-4}$ & $5.948 \times 10^{-3}$  & $6.884 \times 10^{-3}$ & $5.138 \times 10^{-4}$ & $5.812 \times 10^{-3}$ & \colorbox{Dandelion}{${4.738 \times 10^{-5}}$} & \colorbox{Goldenrod}{${4.055 \times 10^{-5}}$} \\
        \textbf{Size} & $66,561$ & $66,561$ & $197,377$ & $66,561$ & $66,561$ & $66,561$ & $66,561$ \\
        \textbf{Train Time(s)} & $0.61$ & $0.87$ & $0.84$ & $0.54$ & $2.31$ & $0.54$ & $0.61$ \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{-10pt}
\end{table}

\par We evaluate audio reconstruction using two-layer models with $256$ neurons in each layer. We used the Spoken English Wikipedia dataset \cite{spokenwikipedia} as a reference, which contains 1,313 clips sampled at $f_\text{s} = 4\,\text{kHz}$, informing a Nyquist frequency of $f_\text{Nyquist} = 2\,\text{kHz}$,. For each clip, we fit the first $10$ seconds of audio and report performance in terms of mean squared error (MSE), averaged across all clips. As summarized in Table~\ref{fig:AudioMse}, FM-SIREN and FM-FINER achieve substantially lower errors than all baselines, and FM-FINER achieves the best overall performance. This demonstrates the effectiveness of Nyquist-informed frequency diversity in capturing fine-grained temporal structures. Figure~\ref{fig:audio-fit} provides qualitative results on a one-second segment of the 1995 Pacific Grand Prix clip, where our models exhibit a markedly lower reconstruction error compared to SIREN, FINER, and other baselines.

